Discovering Polarized Communities in Signed Networks

Signed networks contain edge annotations to indicate whether each interaction is friendly (positive edge) or antagonistic (negative edge). The model is simple but powerful and it can capture novel and interesting structural properties of real-world phenomena. The analysis of signed networks has many applications from modeling discussions in social media, to mining user reviews, and to recommending products in e-commerce sites. In this paper we consider the problem of discovering polarized communities in signed networks. In particular, we search for two communities (subsets of the network vertices) where within communities there are mostly positive edges while across communities there are mostly negative edges. We formulate this novel problem as a "discrete eigenvector" problem, which we show to be NP-hard. We then develop two intuitive spectral algorithms: one deterministic, and one randomized with quality guarantee $\sqrt{n}$ (where $n$ is the number of vertices in the graph), tight up to constant factors. We validate our algorithms against non-trivial baselines on real-world signed networks. Our experiments confirm that our algorithms produce higher quality solutions, are much faster and can scale to much larger networks than the baselines, and are able to detect ground-truth polarized communities.

==> experiments.tex <==
\begin{table*}[t!]
\centering
\caption{\label{tab:evaluation}Solution characterization: communities $S_1$ and $S_2$ (size, number of edges, edge density $d$, ratio of positive edges $\rho_+$, diameter $d\!i\!a\!m$), and between $S_1$ and $S_2$ (number of edges, edge density $d$, ratio of negative edges $\rho_-$).}
% \vspace{-3mm}
\centerline{
\small
\renewcommand{\arraystretch}{0.6}
\newcommand\Tstrut{\rule{0pt}{2.05ex}}
\begin{tabular}{lcrrrrrrrrrrrrr}
\toprule
\multicolumn{2}{c|}{} & \multicolumn{5}{c|}{$S_1$} & \multicolumn{5}{c|}{$S_2$} & \multicolumn{3}{c}{between $S_1$--$S_2$}\\\cline{3-15}
dataset & \multicolumn{1}{c|}{method} & $|S_1|$ & \# edges & $d$ & $\rho_+$ & \multicolumn{1}{r|}{$d\!i\!a\!m$} & $|S_2|$ & \# edges & $d$ & $\rho_+$ & \multicolumn{1}{r|}{$d\!i\!a\!m$} & \# edges & $d$ & $\rho_-$\Tstrut\\
\midrule
\multicolumn{1}{l|}{\textsf{Highland}} & \multicolumn{1}{c|}{\sc E} & $7$    &    $14$    &    $0.33$    &    $1$    &    $2$    &    $4$    &    $6$    &    $0.5$\,\,\, & $1$    &    $1$    &    $14$    &    $0.5$\,\,\,    &    $1$\\
\multicolumn{1}{l|}{\textsf{Tribes}} & \multicolumn{1}{c|}{\sc RE} & $7$    &    $14$    &    $0.33$    &    $1$    &    $2$    &    $4$    &    $6$    &    $0.5$\,\,\, & $1$    &    $1$    &    $14$    &    $0.5$\,\,\,    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $12$    &    $30$    &    $0.22$    &    $0.76$    &    $3$    &    $4$    &    $6$    &    $0.5$\,\,\, & $1$    &    $1$    &    $22$    &    $0.45$    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $4$    &    $6$    &    $0.5$\,\,\, & $1$    &    $1$    &    $5$    &    $3$    &    $0.15$    &    $1$    &    $\infty$    &    $13$    &    $0.65$    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $4$    &    $6$    &    $0.5$\,\,\, & $1$    &    $1$    &    $7$    &    $14$    &    $0.33$    &    $1$    &    $2$    &    $14$    &    $0.5$\,\,\,    &    $1$\\\hline
%
\multicolumn{1}{l|}{\textsf{Cloister}} & \multicolumn{1}{c|}{\sc E} & $3$    &    $3$    &    $0.5$\,\,\, & $1$    &    $1$    &    $8$    &    $22$    &    $0.39$    &    $0.86$    &    $2$    &    $22$    &    $0.91$    &    $1$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $3$    &    $3$    &    $0.5$\,\,\, & $1$    &    $1$    &    $8$    &    $22$    &    $0.39$    &    $0.86$    &    $2$    &    $22$    &    $0.91$    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $3$    &    $3$    &    $0.5$\,\,\, & $1$    &    $1$    &    $15$    &    $80$    &    $0.38$    &    $0.61$    &    $2$    &    $42$    &    $0.93$    &    $0.9$\,\,\,\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $10$    &    $38$    &    $0.42$    &    $0.65$    &    $2$    &    $3$    &    $3$    &    $0.5$\,\,\, & $1$    &    $1$    &    $28$    &    $0.93$    &    $0.89$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $3$    &    $3$    &    $0.5$\,\,\, & $1$    &    $1$    &    $8$    &    $22$    &    $0.39$    &    $0.86$    &    $2$    &    $22$    &    $0.91$    &    $1$\\\hline
%
\multicolumn{1}{l|}{\textsf{Congress}} & \multicolumn{1}{c|}{\sc E} & $28$    &    $73$    &    $0.09$    &    $1$    &    $4$    &    $24$    &    $52$    &    $0.09$    &    $1$    &    $4$    &    $52$    &    $0.07$    &    $0.94$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $45$    &    $106$    &    $0.05$    &    $0.98$    &    $5$    &    $42$    &    $86$    &    $0.04$    &    $1$    &    $\infty$    &    $71$    &    $0.03$    &    $0.9$\,\,\,\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $34$    &    $92$    &    $0.08$    &    $0.98$    &    $5$    &    $37$    &    $95$    &    $0.07$    &    $1$    &    $5$    &    $36$    &    $0.02$    &    $0.77$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $7$    &    $11$    &    $0.26$    &    $1$    &    $2$    &    $5$    &    $6$    &    $0.3$\,\,\, & $1$    &    $3$    &    $11$    &    $0.31$    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $58$    &    $76$    &    $0.02$    &    $0.97$    &    $\infty$    &    $67$    &    $105$    &    $0.02$    &    $1$    &    $6$    &    $61$    &    $0.01$    &    $0.85$\\\hline
%
\multicolumn{1}{l|}{\textsf{Bitcoin}} & \multicolumn{1}{c|}{\sc E} & $2$    &    $0$    &    $0$    &    $0$    &    $\infty$    &    $136$    &    $2\,200$    &    $0.11$    &    $0.95$    &    $3$    &    $45$    &    $0.16$    &    $0.88$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $84$    &    $124$    &    $0.01$    &    $0.99$    &    $\infty$    &    $743$    &    $6\,221$    &    $0.01$    &    $0.95$    &    $5$    &    $678$    &    $0.01$    &    $0.93$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $140$    &    $2\,211$    &    $0.11$    &    $0.95$    &    $3$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $20$    &    $89$    &    $0.23$    &    $1$    &    $2$    &    $21$    &    $20$    &    $0.04$    &    $0.9$\,\,\, & $3$    &    $368$    &    $0.87$    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $398$    &    $163$    &    $1.0e\!-\!03$    &    $0.92$    &    $\infty$    &    $2\,528$    &    $5\,437$    &    $8.5e\!-\!04$    &    $0.95$    &    $\infty$    &    $920$    &    $9.1e\!-\!04$    &    $0.76$\\\hline
%
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $745$    &    $31\,247$    &    $0.05$    &    $0.92$    &    $3$    &    $3$    &    $0$    &    $0$    &    $0$    &    $\infty$    &    $219$    &    $0.09$    &    $0.83$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Elections}} & \multicolumn{1}{c|}{\sc RE} & $1\,014$    &    $36\,334$    &    $0.03$    &    $0.91$    &    $4$    &    $53$    &    $4$    &    $1.4e\!-\!03$    &    $0$    &    $\infty$    &    $891$    &    $0.01$    &    $0.8$\,\,\,\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $731$    &    $31\,181$    &    $0.05$    &    $0.92$    &    $3$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $408$    &    $10\,588$    &    $0.06$    &    $0.88$    &    $2$    &    $7$    &    $1$    &    $0.02$    &    $0$    &    $\infty$    &    $114$    &    $0.03$    &    $0.89$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $2\,804$    &    $24\,209$    &    $3.0e\!-\!03$    &    $0.88$    &    $\infty$    &    $801$    &    $232$    &    $3.6e\!-\!04$    &    $0.35$    &    $\infty$    &    $3\,941$    &    $1.7e\!-\!03$    &    $0.73$\\\hline
%
\multicolumn{1}{l|}{\textsf{Referendum}} & \multicolumn{1}{c|}{\sc E} & $669$    &    $57\,990$    &    $0.12$    &    $1$    &    $2$    &    $4$    &    $5$    &    $0.41$    &    $1$    &    $2$    &    $1\,022$    &    $0.38$    &    $0.78$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $1\,477$    &    $90\,694$    &    $0.04$    &    $0.99$    &    $4$    &    $17$    &    $23$    &    $0.08$    &    $1$    &    $4$    &    $1\,803$    &    $0.07$    &    $0.74$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $685$    &    $59\,574$    &    $0.12$    &    $1$    &    $2$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $1\,143$    &    $67\,511$    &    $0.05$    &    $1$    &    $2$    &    $16$    &    $30$    &    $0.12$    &    $1$    &    $2$    &    $1\,587$    &    $0.08$    &    $0.79$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $527$    &    $1\,633$    &    $5.8e\!-\!03$    &    $1$    &    $\infty$    &    $4\,988$    &    $66\,843$    &    $2.6e\!-\!03$    &    $0.99$    &    $\infty$    &    $7\,839$    &    $2.9e\!-\!03$    &    $0.4$\,\,\,\\\hline
%
\multicolumn{1}{l|}{\textsf{Slashdot}} & \multicolumn{1}{c|}{\sc E} & $233$    &    $9\,550$    &    $0.17$    &    $0.98$    &    $3$    &    $1$    &    $0$    &    $0$    &    $0$    &    $0$    &    $34$    &    $0.14$    &    $0.94$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $2\,854$    &    $49\,037$    &    $6.0e\!-\!03$ &$0.93$    &    $5$    &    $112$    &    $65$    &    $5.2e\!-\!03$    &    $0.23$    &    $\infty$    &    $2\,630$    &    $8.2e\!-\!03$    &    $0.81$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $200$    &    $8\,486$    &    $0.21$    &    $0.98$    &    $2$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $284$    &    $9\,276$    &    $0.11$    &    $0.99$    &    $2$    &    $6$    &    $1$    &    $0.03$    &    $1$    &    $\infty$    &    $197$    &    $0.11$    &    $0.51$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $35\,099$    &    $109\,899$    &    $8.9e\!-\!05$    &    $0.87$    &    $\infty$    &    $5\,766$    &    $2\,264$    &    $6.8e\!-\!05$    &    $0.48$    &    $\infty$    &    $22\,404$    &    $1.1e\!-\!04$    &    $0.7$\,\,\,\\\hline
%
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $1\,993$    &    $155\,278$    &    $0.03$    &    $0.91$    &    $3$    &    $449$    &    $13$    &    $6.4e\!-\!05$    &    $0$    &    $\infty$    &        $84\,280$    &    $0.09$    &    $0.99$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Conflict}} & \multicolumn{1}{c|}{\sc RE} & $9\,603$    &    $397\,092$    &    $4.3e\!-\!03$    &    $0.89$    &    $4$    &    $3\,085$    &    $370$    &    $3.8e\!-\!05$    &    $0.01$    &    $\infty$    &    $331\,400$    &    $0.01$    &    $0.99$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $1\,159$    &    $79\,644$    &    $0.05$    &    $0.96$    &    $3$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $369$    &    $16\,760$    &    $0.12$    &    $0.96$    &    $2$    &    $134$    &    $941$    &    $0.05$    &    $2.1e\!-\!03$    &    $4$    &    $19\,928$    &    $0.4$\,\,\,    &    $0.96$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $23\,972$    &    $240\,615$    &    $4.1e\!-\!04$    &    $0.84$    &    $\infty$    &    $34\,448$    &    $3\,929$    &    $3.3e\!-\!06$    &    $0.06$    &    $\infty$    &    $287\,512$    &    $3.4e\!-\!04$    &    $0.99$\\\hline
%
\multicolumn{1}{l|}{\textsf{Epinions}} & \multicolumn{1}{c|}{\sc E} & $999$    &    $69\,636$    &    $0.06$    &    $0.95$    &    $3$    &    $18$    &    $24$    &    $0.07$    &    $0.41$    &    $\infty$    &    $2\,903$    &    $0.16$    &    $0.85$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $4\,050$    &    $171\,647$    &    $0.01$    &    $0.94$    &    $\infty$    &    $384$    &    $236$    &    $1.6e\!-\!03$    &    $0.47$    &    $\infty$    &    $12\,243$    &    $7.8e\!-\!03$    &    $0.87$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $269$    &    $22\,919$    &    $0.31$    &    $0.99$    &    $2$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $249$    &    $19\,786$    &    $0.32$    &    $0.99$    &    $2$    &    $5$    &    $2$    &    $0.1$\,\,\, & $1$    &    $\infty$    &    $259$    &    $0.2$\,\,\,    &    $1$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $49\,402$    &    $151\,424$    &    $6.2e\!-\!05$    &    $0.94$    &    $\infty$    &    $16\,608$    &    $3\,253$    &    $1.1e\!-\!05$    &    $0.78$    &    $\infty$    &    $26\,237$    &    $3.1e\!-\!05$    &    $0.76$\\\hline
%
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $2$    &    $1$    &    $0.5$    &    $0$    &    $1$    &    $646$    &    $30\,764$    &    $0.07$    &    $0.96$    &    $3$    &    $102$    &    $0.07$    &    $1$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Politics}} & \multicolumn{1}{c|}{\sc RE} & $513$    &    $277$    &    $1.0e\!-\!03$    &    $0.23$    &    $\infty$    &    $6\,769$    &    $141\,249$    &    $3.0e\!-\!03$    &    $0.95$    &    $5$    &    $3\,917$    &    $1.1e\!-\!03$    &    $0.82$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $543$    &    $26\,059$    &    $0.088$    &    $0.96$    &    $3$    &    $0$    &    $0$    &    $0$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $599$    &    $15\,370$    &    $0.04$    &    $0.98$    &    $2$    &    $11$    &    $0$    &    $0$    &    $0$    &    $\infty$    &    $242$    &    $0.03$    &    $0.4$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $18\,990$    &    $8\,068$    &    $2.2e\!-\!05$    &    $0.79$    &    $\infty$    &    $50\,371$    &    $159\,711$    &    $6.2e\!-\!05$    &    $0.95$    &    $\infty$    &    $20\,748$    &    $2.1e\!-\!05$    &    $0.68$\\
\bottomrule
\end{tabular}
}
\end{table*}


\spara{Baselines.}


\spara{Comparative evaluation.}


To take a deeper look into the quality of the solutions, beyond the value of \score and the size, we report in Figure~\ref{fig:quality} the ratios of positive edges within the two communities and the ratio of negative edges in-between.
We refer to the two communities included in the solutions as $S_1$ and $S_2$, namely the subsets of vertices that are assigned with $1$ and $-1$, respectively, by the solution vector $\vec{x}$.
Community $S_1$ has high ratio of positive edges, close to the maximum, in most of the datasets for all algorithms.
On the other hand, the results are different for community $S_2$.
% For \textsf{College}, for example, none of the algorithms is able to find a cohesive second community.
For \textsf{Referendum} and \textsf{Epinions}, instead, algorithm {\sc G} is the only method unable to identify two positive-dense subsets of vertices.
With regards to the negative ratio, for \textsf{HighlandTribes}, \textsf{Cloister}, and \textsf{Congress}, all algorithms return solutions having high portion of negative edges between $S_1$ and $S_2$.
It is important to notice that for the larger datasets, from \textsf{Bitcoin} to \textsf{WikiPolitics}, algorithm {\sc G} is the only method having negative ratio always equal to $0$.
This testifies that algorithm {\sc G}, albeit can output solutions of high \scoreshort, fails to identify an actual pair of polarized communities, rather it discovers communities with only high internal density.
Therefore, algorithm {\sc G} finds structures not suitable for our purpose.
Finally, note that finding a solution having $S_1$ or $S_2$ with no positive edges within, yet with negative edges towards the other community is allowed by our formulation of the problem.
It has to be further investigate whether \ourproblem favors such solutions over polarized structures.

\begin{figure}[t!]
\centerline{
\includegraphics[width=1.1\columnwidth]{figures/evaluation_runtime.pdf}
}
% \vspace{-3mm}
\caption{\label{fig:evaluation_runtime} Runtime: proposed algorithms and baselines.}
\end{figure}

\begin{figure}[t!]
\centerline{
\includegraphics[width=1.1\columnwidth]{figures/evaluation_scalability.pdf}
}
% \vspace{-3mm}
\caption{\label{fig:evaluation_scalability} Scalability: runtime of the proposed algorithms as a function of number of injected noisy vertices for \textsf{Slashdot}, \textsf{WikiConflict}, \textsf{Epinions}, and \textsf{WikiPolitics}.}
\end{figure}

\spara{Runtime and scalability.}
To assess the advantages of our algorithms in terms of efficiency, we show in Figure~\ref{fig:evaluation_runtime} their runtime compared to the baselines.
Both algorithms {\sc E} and {\sc RE} terminate in less than a $40$ seconds for all datasets.
The practical enhancements do not heavily contribute to the execution time.
In particular, the evaluation of $\tau$ in algorithm {\sc E} is carried out efficiently, since $\vec{v}$ is computed only once regardless of the number of considered values of threshold.
On the other hand, algorithm {\sc G} is extremely demanding in terms of running time: algorithms {\sc E} and {\sc RE} are faster than algorithm {\sc G} of more than an order magnitude for the larger datasets (i.e., \textsf{Slashdot}, \textsf{WikiConflict}, \textsf{Epinions}, and \textsf{WikiPolitics}).
The runtime of algorithms {\sc B} and {\sc LS} is comparable to algorithm {\sc G}, thus more than an order of magnitude higher than algorithms {\sc E} and {\sc RE}.

The proposed algorithms are also able to efficiently scale to datasets of huge dimension.
To prove this property, we augment the larger datasets (i.e., \textsf{Slashdot}, \textsf{WikiConflict}, \textsf{Epinions}, and \textsf{WikiPolitics}) from $|V| / 2$ to $16|V|$ random vertices by the same methodology described above.
As a result, we obtain datasets composed of up to $2.3$\,M vertices (\textsf{WikiPolitics} augmented with $16|V|$ noisy vertices) and $67.3$\,M edges (\textsf{WikiConflict} augmented with $16|V|$ noisy vertices).
Note that, as the quantity of noise increases, $\delta$, i.e., the ratio of non-zero elements of the adjacency matrix, decreases.
Nonetheless, $\delta$ differs with respect to the original datasets less than an order of magnitude in all cases, making the following results about scalability significant.
As shown in Figure~\ref{fig:evaluation_scalability}, that reports the runtime of algorithms {\sc E} and {\sc RE} as a function of the number of injected random vertices, the time required by both our methods, in practice, grows linearly with the number of vertices.
Among the two, algorithm {\sc E} is slightly slower than algorithm {\sc RE} due to the evaluation of multiple values of the threshold $\tau$.
In the worst case, Algorithms {\sc E} returns in about $21$ minutes.

\spara{Case study.}






\iffalse
\begin{figure}[t!]
\centerline{
\includegraphics[width=1.1\columnwidth]{figures/evaluation_quality.pdf}
}
%\vspace{-3mm}
\caption{\label{fig:quality} Edge ratios: ratio of positive edges within $S_1$ (top), ratio of positive edges within $S_2$ (middle), and ratio of negative edge between $S_1$ and $S_2$ (bottom).}
\end{figure}

\begin{figure}[t!]
\centerline{
\includegraphics[width=1.1\columnwidth]{figures/evaluation_noised.pdf}
}
%\vspace{-3mm}
\caption{\label{fig:noise} \score comparison with random noise for \textsf{HighlandTribes}, \textsf{Cloister}, \textsf{College}, and \textsf{Congress}.
The labels on the $x$-axes refer to the number of injected noisy vertices.}
\end{figure}

\spara{Random noise.}
To evaluate the ability of our algorithms to find planted polarized communities, we artificially augment the smaller datasets with random noise.
In particular, we incrementally inject into each dataset noisy vertices having number of randomly-connected edges equal to the average degree of the original network.
Moreover, we maintain the ratio of negative edges.
Figure~\ref{fig:noise} shows the \score of the solutions output by our algorithms and the baselines for \textsf{HighlandTribes}, \textsf{Cloister}, \textsf{College}, and \textsf{Congress} augmented from $|V| / 2$ to $16|V|$ noisy vertices.
For each quantity of noise, we reproduce the injection ten times, i.e., we create ten different augmented networks, and we report the average \scoreshort.

The superiority of our algorithms is visible in all cases, with algorithm {\sc E} always leading the baselines.
As the quantity of noise increases, the baselines become less competitive, especially for \textsf{HighlandTribes}.
The only exception is \textsf{College}, in which algorithm {\sc G} has \score comparable to algorithms {\sc E} and {\sc RE} up to $16|V|$ noisy vertices, probably, due to the lack of a 2-polarized-communities structure in the original dataset.
We also experiment the addition of noisy vertices to the larger dataset without noting any evident difference with respect to the original cases.
\fi

\iffalse
\multicolumn{1}{l|}{\textsf{Highland}} & \multicolumn{1}{c|}{\sc E} & $6.18$    &    $7$    &    $28$    &    $28$    &    $4$    &    $12$    &    $12$    &    $14$    &    $14$    &    $0.005$\\
\multicolumn{1}{l|}{\textsf{Tribes}} & \multicolumn{1}{c|}{\sc RE} & $6.16$    &    $8$    &    $32$    &    $32$    &    $4$    &    $12$    &    $12$    &    $15$    &    $15$    &    $0.004$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $5.5$    &    $12$    &    $60$    &    $46$    &    $4$    &    $12$    &    $12$    &    $22$    &    $22$    &    $0.005$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $4.88$    &    $4$    &    $12$    &    $12$    &    $5$    &    $6$    &    $6$    &    $13$    &    $13$    &    $0.001$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $6.18$    &    $4$    &    $12$    &    $12$    &    $7$    &    $28$    &    $28$    &    $14$    &    $14$    &    $0.002$\\\hline
\multicolumn{1}{l|}{\textsf{Cloister}} & \multicolumn{1}{c|}{\sc E} & $7.45$    &    $3$    &    $6$    &    $6$    &    $8$    &    $44$    &    $38$    &    $22$    &    $22$    &    $0.004$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $7.07$    &    $3$    &    $6$    &    $6$    &    $10$    &    $64$    &    $48$    &    $27$    &    $27$    &    $0.015$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $6.11$    &    $3$    &    $6$    &    $6$    &    $15$    &    $160$    &    $98$    &    $42$    &    $38$    &    $0.013$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $5.69$    &    $10$    &    $76$    &    $50$    &    $3$    &    $6$    &    $6$    &    $28$    &    $25$    &    $0.002$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $7.45$    &    $3$    &    $6$    &    $6$    &    $8$    &    $44$    &    $38$    &    $22$    &    $22$    &    $0.003$\\\hline
\multicolumn{1}{l|}{\textsf{Congress}} & \multicolumn{1}{c|}{\sc E} & $6.57$    &    $28$    &    $146$    &    $146$    &    $24$    &    $104$    &    $104$    &    $52$    &    $49$    &    $0.078$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $5.59$    &    $46$    &    $232$    &    $228$    &    $43$    &    $172$    &    $172$    &    $61$    &    $56$    &    $0.03$\,\,\,\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $5.77$    &    $34$    &    $184$    &    $182$    &    $37$    &    $190$    &    $190$    &    $36$    &    $28$    &    $0.015$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $4.66$    &    $7$    &    $22$    &    $22$    &    $5$    &    $12$    &    $12$    &    $11$    &    $11$    &    $0.01$\,\,\,\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $3.01$    &    $53$    &    $134$    &    $134$    &    $48$    &    $108$    &    $106$    &    $49$    &    $41$    &    $0.015$\\\hline
\multicolumn{1}{l|}{\textsf{Bitcoin}} & \multicolumn{1}{c|}{\sc E} & $29.52$    &    $2$    &    $0$    &    $0$    &    $136$    &    $4\,400$    &    $4\,202$    &    $45$    &    $40$    &    $1.293$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $14.89$    &    $80$    &    $194$    &    $194$    &    $726$    &    $11\,902$    &    $11\,302$    &    $601$    &    $578$    &    $0.449$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $29.01$    &    $0$    &    $0$    &    $0$    &    $140$    &    $4\,422$    &    $4\,242$    &    $0$    &    $0$    &    $1.835$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $23.07$    &    $20$    &    $178$    &    $178$    &    $21$    &    $40$    &    $36$    &    $368$    &    $368$    &    $1.135$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $3.46$    &    $2\,573$    &    $10\,146$    &    $9\,610$    &    $386$    &    $218$    &    $208$    &    $863$    &    $678$    &    $1.851$\\\hline
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $71.73$    &    $745$    &    $62\,494$    &    $57\,928$    &    $3$    &    $0$    &    $0$    &    $219$    &    $183$    &    $2.231$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Elections}} & \multicolumn{1}{c|}{\sc RE} & $56.63$    &    $1\,019$    &    $73\,114$    &    $66\,764$    &    $72$    &    $26$    &    $6$    &    $1\,137$    &    $917$    &    $1.203$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $72.67$    &    $731$    &    $62\,362$    &    $57\,742$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $4.793$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $39.49$    &    $408$    &    $21\,176$    &    $18\,694$    &    $7$    &    $2$    &    $0$    &    $114$    &    $102$    &    $3.903$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $10.221$    &    $2\,780$    &    $45\,284$    &    $39\,314$    &    $836$    &    $466$    &    $184$    &    $4\,114$    &    $2\,993$    &    $5.582$\\\hline
\multicolumn{1}{l|}{\textsf{Referendum}} & \multicolumn{1}{c|}{\sc E} & $174.08$    &    $669$    &    $115\,980$    &    $115\,980$    &    $4$    &    $10$    &    $10$    &    $1\,022$    &    $803$    &    $4$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $120.82$    &    $1\,512$    &    $182\,778$    &    $182\,774$    &    $16$    &    $40$    &    $40$    &    $1\,787$    &    $1\,345$    &    $2$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $173.93$    &    $685$    &    $119\,148$    &    $119\,148$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $24$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $118.15$    &    $1\,143$    &    $135\,022$    &    $135\,022$    &    $16$    &    $60$    &    $60$    &    $1\,587$    &    $1\,257$    &    $20$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $23.86$    &    $527$    &    $3\,266$    &    $3\,266$    &    $4\,988$    &    $133\,686$    &    $132\,554$    &    $7\,839$    &    $3\,147$    &    $157$\\\hline
\multicolumn{1}{l|}{\textsf{Slashdot}} & \multicolumn{1}{c|}{\sc E} & $79.69$    &    $233$    &    $19\,100$    &    $18\,844$    &    $1$    &    $0$    &    $0$    &    $34$    &    $32$    &    $21$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $29.93$    &    $2\,900$    &    $99\,482$    &    $93\,126$    &    $96$    &    $72$    &    $26$    &    $2\,167$    &    $1\,814$    &    $8$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $82.72$    &    $200$    &    $16\,972$    &    $16\,758$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $657$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $62.74$    &    $284$    &    $18\,552$    &    $18\,368$    &    $6$    &    $2$    &    $2$    &    $197$    &    $101$    &    $493$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $4.44$    &    $35\,099$    &    $219\,798$    &    $191\,420$    &    $5\,766$    &    $4\,528$    &    $2\,174$    &    $22\,404$    &    $15\,869$    &    $389$\\\hline
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $175.65$    &    $1\,993$    &    $310\,556$    &    $285\,562$    &    $449$    &    $26$    &    $0$    &    $84\,280$    &    $84\,241$    &    $37$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Conflict}} & \multicolumn{1}{c|}{\sc RE} & $101.66$    &    $9\,665$    &    $798\,690$    &    $717\,926$    &    $3\,081$    &    $648$    &    $18$    &    $330\,983$    &    $330\,319$    &    $23$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $127.97$    &    $1\,159$    &    $159\,288$    &    $153\,806$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $1\,857$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $131.07$    &    $369$    &    $33\,520$    &    $32\,202$    &    $134$    &    $1\,882$    &    $4$    &    $19\,928$    &    $19\,194$    &    $1\,968$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $15.23$    &    $23\,972$    &    $481\,230$    &    $406\,162$    &    $34\,448$    &    $7\,858$    &    $532$    &    $287\,512$    &    $285\,169$    &    $5\,402$\\\hline
\multicolumn{1}{l|}{\textsf{Epinions}} & \multicolumn{1}{c|}{\sc E} & $128.72$    &    $999$    &    $139\,272$    &    $133\,024$    &    $18$    &    $48$    &    $20$    &    $2\,903$    &    $2\,487$    &    $26$\Tstrut\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc RE} & $73.18$    &    $3\,949$    &    $333\,600$    &    $316\,586$    &    $385$    &    $462$    &    $214$    &    $11\,797$    &    $10\,308$    &    $11$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $170.29$    &    $269$    &    $45\,838$    &    $45\,824$    &    $0$    &    $0$    &    $0$    &    $0$    &    $0$    &    $1\,793$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $157.75$    &    $249$    &    $39\,572$    &    $39\,560$    &    $5$    &    $4$    &    $4$    &    $259$    &    $259$    &    $964$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $4.55$    &    $49\,402$    &    $302\,848$    &    $285\,842$    &    $16\,608$    &    $6\,506$    &    $5\,088$    &    $26\,237$    &    $20\,175$    &    $857$\\\hline
\multicolumn{1}{l|}{\textsf{Wiki}} & \multicolumn{1}{c|}{\sc E} & $88.44$    &    $2$    &    $2$    &    $0$    &    $646$    &    $61\,528$    &    $59\,318$    &    $102$    &    $102$    &    $30$\Tstrut\\
\multicolumn{1}{l|}{\textsf{Politics}} & \multicolumn{1}{c|}{\sc RE} & $35.88$    &    $538$    &    $666$    &    $184$    &    $6\,884$    &    $285\,394$    &    $273\,350$    &    $4\,290$    &    $3\,470$    &    $13$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc G} & $90.02$    &    $0$    &    $0$    &    $0$    &    $543$    &    $52\,118$    &    $50\,500$    &    $0$    &    $0$    &    $1\,715$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc B} & $48.44$    &    $599$    &    $30\,740$    &    $30\,190$    &    $11$    &    $0$    &    $0$    &    $242$    &    $99$    &    $1\,136$\\
\multicolumn{1}{l|}{} & \multicolumn{1}{c|}{\sc LS} & $4.52$    &    $18\,990$    &    $16\,136$    &    $12\,758$    &    $50\,371$    &    $319\,422$    &    $304\,392$    &    $20\,748$    &    $14\,190$    &    $792$\\
\fi 
